JURY-RL: Votes Propose, Proofs Dispose for Label-Free RLVR

Reinforcement learning with verifiable rewards (RLVR) enhances the reasoning of large language models (LLMs), but standard RLVR often depends on human-annotated answers or carefully curated reward specifications. In machine-checkable domains, label-free alternatives such as majority voting or LLM-as-a-judge remove annotation cost but can introduce false positives that destabilize training. We introduce JURY-RL, a label-free RLVR framework that decouples answer proposal from reward disposal: votes from model rollouts propose a candidate answer, and a formal verifier determines whether that candidate can receive positive reward. Concretely, only rollouts matching the plurality-voted answer are rewarded when that answer is successfully verified in Lean. When verification is inconclusive, we invoke ResZero (Residual-Zero), a fallback reward that discards the unverified plurality proposal and redistributes a zero-mean, variance-preserving signal over the residual answers. This design maintains a stable optimization gradient without reinforcing unverifiable consensus. Across three backbone models trained on mathematical data, JURY-RL consistently outperforms other label-free baselines on mathematical reasoning benchmarks and transfers competitively to code generation and general benchmarks. It attains pass@1 performance comparable to supervised ground-truth training, with superior generalization demonstrated by higher pass@k and response diversity.

==> Table/main_result_pass1.tex <==

% \begin{table*}[!t]
%     \centering
%     \caption{Main Results (\%) of \textit{RL performance} comparison on math reasoning benchmarks. Cell background colors indicate relative performance: darker colors denote better results within each model group.  
%     }
%     \renewcommand{\arraystretch}{1.05}
%     \label{tab:main_math}
%     \vspace{2mm}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|rrcccrcccc}
%     \toprule[1.6pt]
%         \multirow{2}*{\textbf{Methods}} & \multicolumn{5}{c}{\textbf{Mathematics}} & \multicolumn{2}{c}{\textbf{Code}} & \textbf{Instruction} & \textbf{Multi-Task} & \multirow{2}*{\textbf{Average}} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10}

%         ~ & \textbf{AIME24} & \textbf{AIME25} & \textbf{MATH500} & \textbf{GSM8K} & \textbf{AMC} & \textbf{LiveCode} & \textbf{CRUX} & \textbf{IFEval} & \textbf{MMLU-Pro} &  ~ \\
%         \midrule
%             \multicolumn{11}{c}{\textit{\textbf{Qwen3-1.7B-Base}}} \\ 
%         \midrule

%         Before RL & $6.67_{\, \pm 4.6}$ & $6.67_{\, \pm 4.6}$ & $45.8_{\, \pm 2.2}$ & $63.31_{\, \pm 1.3}$ & $26.51_{\, \pm 4.8}$ & $4.59_{\, \pm 0.4}$ & $7.12_{\, \pm 0.9}$ & $33.66_{\, \pm 1.0}$ & $33.60_{\, \pm 0.4}$ & $25.33_{\, \pm 2.3}$ \\
%         GT-Reward & $10.00_{\, \pm 5.6}$ & $0.00_{\, \pm 0.0}$ & $68.2_{\, \pm 2.1}$ & $83.09_{\, \pm 1.0}$ & $34.94_{\, \pm 5.2}$ & $14.84_{\, \pm 0.9}$ & $33.75_{\, \pm 1.7}$ & $38.70_{\, \pm 1.0}$ & $39.43_{\, \pm 0.4}$ & $35.88_{\, \pm 2.0}$ \\
%         \midrule
%         Self-Certainty & \cellcolor{lightpurple3}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple1}{$57.2_{\, \pm 2.2}$} & \cellcolor{lightpurple1}{$74.68_{\, \pm 1.2}$} & \cellcolor{lightpurple1}{$26.51_{\, \pm 4.8}$} & \cellcolor{lightblue1}{$10.37_{\, \pm 0.7}$} & \cellcolor{lightblue1}{$19.00_{\, \pm 1.4}$} & \cellcolor{lightblue7}{$38.58_{\, \pm 1.0}$} & \cellcolor{lightblue2}{$35.28_{\, \pm 0.4}$} & \cellcolor{tealgreen1}{$30.18_{\, \pm 2.2}$} \\
%         Entropy & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple4}{$65.2_{\, \pm 2.1}$} & \cellcolor{lightpurple2}{$79.98_{\, \pm 1.1}$} & \cellcolor{lightpurple3}{$32.53_{\, \pm 5.1}$} & \cellcolor{lightblue2}{$12.64_{\, \pm 0.8}$} & \cellcolor{lightblue2}{$31.00_{\, \pm 1.6}$} & \cellcolor{lightblue2}{$35.00_{\, \pm 1.0}$} & \cellcolor{lightblue4}{$37.01_{\, \pm 0.4}$} & \cellcolor{tealgreen3}{$34.08_{\, \pm 2.4}$} \\
%         Majority-Voting & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple1}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple2}{$59.8_{\, \pm 2.2}$} & \cellcolor{lightpurple4}{$81.88_{\, \pm 1.1}$} & \cellcolor{lightpurple4}{$33.73_{\, \pm 5.2}$} & \cellcolor{lightblue5}{$14.29_{\, \pm 0.9}$} & \cellcolor{lightblue4}{$32.75_{\, \pm 1.7}$} & \cellcolor{lightblue5}{$37.16_{\, \pm 1.0}$} & \cellcolor{lightblue3}{$35.68_{\, \pm 0.4}$} & \cellcolor{tealgreen2}{$33.18_{\, \pm 1.8}$} \\
%         CoReward & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple5}{$66.0_{\, \pm 2.1}$} & \cellcolor{lightpurple5}{$82.03_{\, \pm 1.1}$} & \cellcolor{lightpurple4}{$33.73_{\, \pm 5.2}$} & \cellcolor{lightblue4}{$14.27_{\, \pm 0.9}$} & \cellcolor{lightblue3}{$32.12_{\, \pm 1.6}$} & \cellcolor{lightblue6}{$37.28_{\, \pm 1.0}$} & \cellcolor{lightblue5}{$37.39_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$35.13_{\, \pm 2.4}$} \\
%         LLM-KD & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple7}{$68.4_{\, \pm 2.1}$} & \cellcolor{lightpurple6}{$82.41_{\, \pm 1.1}$} & \cellcolor{lightpurple7}{$44.58_{\, \pm 5.5}$} & \cellcolor{lightblue3}{$14.05_{\, \pm 0.9}$} & \cellcolor{lightblue5}{$34.62_{\, \pm 1.7}$} & \cellcolor{lightblue1}{$34.65_{\, \pm 1.0}$} & \cellcolor{lightblue6}{$37.97_{\, \pm 0.4}$} & \cellcolor{tealgreen6}{$35.93_{\, \pm 2.1}$} \\
%         LLM-as-a-Judge  & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple3}{$62.8_{\, \pm 2.2}$} & \cellcolor{lightpurple3}{$80.52_{\, \pm 1.1}$} & \cellcolor{lightpurple2}{$31.33_{\, \pm 5.1}$} & \cellcolor{lightblue6}{$14.33_{\, \pm 0.9}$} & \cellcolor{lightblue7}{$36.12_{\, \pm 1.7}$} & \cellcolor{lightblue3}{$36.28_{\, \pm 1.0}$} & \cellcolor{lightblue1}{$33.83_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$34.28_{\, \pm 2.4}$} \\
%         \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple7}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple7}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple7}{$68.4_{\, \pm 2.1}$} & \cellcolor{lightpurple7}{$83.32_{\, \pm 1.0}$} & \cellcolor{lightpurple6}{$36.14_{\, \pm 5.3}$} & \cellcolor{lightblue7}{$14.54_{\, \pm 0.9}$} & \cellcolor{lightblue6}{$35.00_{\, \pm 1.7}$} & \cellcolor{lightblue4}{$36.55_{\, \pm 1.0}$} & \cellcolor{lightblue7}{$38.11_{\, \pm 0.4}$} & \cellcolor{tealgreen7}{$36.90_{\, \pm 2.6}$} \\
%         \specialrule{1pt}{0.4ex}{0.4ex}
%             \multicolumn{11}{c}{\textit{\textbf{Llama-3.2-3B-Instruct}}} \\ 
%         \midrule

%         Before RL & $3.33_{\, \pm 3.3}$ & $0.00_{\, \pm 0.0}$ & $42.8_{\, \pm 2.2}$ & $69.75_{\, \pm 1.3}$ & $13.25_{\, \pm 3.7}$ & $3.00_{\, \pm 0.4}$ & $25.50_{\, \pm 1.5}$ & $54.41_{\, \pm 1.1}$ & $32.01_{\, \pm 0.4}$ & $27.12_{\, \pm 1.6}$ \\
%         GT-Reward & $13.33_{\, \pm 6.3}$ & $0.00_{\, \pm 0.0}$ & $48.0_{\, \pm 2.2}$ & $76.72_{\, \pm 1.2}$ & $22.89_{\, \pm 4.6}$ & $7.05_{\, \pm 0.6}$ & $32.62_{\, \pm 1.7}$ & $50.16_{\, \pm 1.1}$ & $34.26_{\, \pm 0.4}$ & $31.67_{\, \pm 2.0}$ \\
%         \midrule
%         Entropy & \cellcolor{lightpurple2}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple1}{$45.0_{\, \pm 2.2}$} & \cellcolor{lightpurple2}{$76.35_{\, \pm 1.2}$} & \cellcolor{lightpurple1}{$19.28_{\, \pm 4.3}$} & \cellcolor{lightblue2}{$4.74_{\, \pm 0.5}$} & \cellcolor{lightblue1}{$23.75_{\, \pm 1.5}$} & \cellcolor{lightblue7}{$56.32_{\, \pm 1.1}$} & \cellcolor{lightblue3}{$33.68_{\, \pm 0.4}$} & \cellcolor{tealgreen2}{$29.53_{\, \pm 1.8}$} \\
%         Self-Certainty & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple1}{$45.0_{\, \pm 2.2}$} & \cellcolor{lightpurple1}{$74.91_{\, \pm 1.2}$} & \cellcolor{lightpurple5}{$21.69_{\, \pm 4.5}$} & \cellcolor{lightblue2}{$4.74_{\, \pm 0.5}$} & \cellcolor{lightblue2}{$26.62_{\, \pm 1.6}$} & \cellcolor{lightblue6}{$55.08_{\, \pm 1.1}$} & \cellcolor{lightblue2}{$33.32_{\, \pm 0.4}$} & \cellcolor{tealgreen1}{$29.41_{\, \pm 1.6}$} \\
%         Majority-Voting & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple3}{$47.0_{\, \pm 2.2}$} & \cellcolor{lightpurple5}{$79.08_{\, \pm 1.1}$} & \cellcolor{lightpurple1}{$19.28_{\, \pm 4.3}$} & \cellcolor{lightblue7}{$8.11_{\, \pm 0.7}$} & \cellcolor{lightblue4}{$31.87_{\, \pm 1.6}$} & \cellcolor{lightblue1}{$48.36_{\, \pm 1.1}$} & \cellcolor{lightblue4}{$33.94_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$30.85_{\, \pm 1.9}$} \\
%         CoReward & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple6}{$49.2_{\, \pm 2.2}$} & \cellcolor{lightpurple6}{$79.76_{\, \pm 1.1}$} & \cellcolor{lightpurple3}{$20.48_{\, \pm 4.4}$} & \cellcolor{lightblue4}{$5.57_{\, \pm 0.5}$} & \cellcolor{lightblue3}{$30.38_{\, \pm 1.6}$} & \cellcolor{lightblue4}{$50.46_{\, \pm 1.1}$} & \cellcolor{lightblue1}{$32.95_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$30.98_{\, \pm 1.9}$} \\
%         LLM-KD & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple7}{$49.4_{\, \pm 2.2}$} & \cellcolor{lightpurple4}{$78.47_{\, \pm 1.1}$} & \cellcolor{lightpurple3}{$20.48_{\, \pm 4.4}$} & \cellcolor{lightblue6}{$7.55_{\, \pm 0.6}$} & \cellcolor{lightblue5}{$32.38_{\, \pm 1.6}$} & \cellcolor{lightblue2}{$49.06_{\, \pm 1.1}$} & \cellcolor{lightblue5}{$34.04_{\, \pm 0.4}$} & \cellcolor{tealgreen5}{$31.26_{\, \pm 1.9}$} \\
%         LLM-as-a-Judge  & \cellcolor{lightpurple2}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple4}{$47.8_{\, \pm 2.2}$} & \cellcolor{lightpurple3}{$77.10_{\, \pm 1.2}$} & \cellcolor{lightpurple5}{$21.69_{\, \pm 4.5}$} & \cellcolor{lightblue1}{$3.96_{\, \pm 0.4}$} & \cellcolor{lightblue7}{$33.88_{\, \pm 1.7}$} & \cellcolor{lightblue5}{$51.46_{\, \pm 1.1}$} & \cellcolor{lightblue6}{$34.22_{\, \pm 0.4}$} & \cellcolor{tealgreen3}{$30.75_{\, \pm 1.8}$} \\
%         \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple7}{$16.67_{\, \pm 6.9}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple5}{$49.0_{\, \pm 2.2}$} & \cellcolor{lightpurple7}{$80.74_{\, \pm 1.1}$} & \cellcolor{lightpurple7}{$24.10_{\, \pm 4.7}$} & \cellcolor{lightblue5}{$6.16_{\, \pm 0.6}$} & \cellcolor{lightblue6}{$32.62_{\, \pm 1.7}$} & \cellcolor{lightblue3}{$50.09_{\, \pm 1.1}$} & \cellcolor{lightblue7}{$34.54_{\, \pm 0.4}$} & \cellcolor{tealgreen7}{$32.66_{\, \pm 2.1}$} \\
%         \specialrule{1pt}{0.4ex}{0.4ex}
%             \multicolumn{11}{c}{\textit{\textbf{Qwen2.5-7B}}} \\ 
%         \midrule

%         Before RL & $3.33_{\, \pm 3.3}$ & $3.33_{\, \pm 3.3}$ & $49.2_{\, \pm 2.2}$ & $71.65_{\, \pm 1.2}$ & $20.48_{\, \pm 4.4}$ & $4.57_{\, \pm 0.4}$ & $28.00_{\, \pm 1.6}$ & $40.61_{\, \pm 1.0}$ & $44.03_{\, \pm 0.4}$ & $29.47_{\, \pm 2.0}$ \\
%         GT-Reward & $13.33_{\, \pm 6.3}$ & $6.67_{\, \pm 4.6}$ & $76.4_{\, \pm 1.9}$ & $89.61_{\, \pm 0.8}$ & $46.99_{\, \pm 5.5}$ & $12.78_{\, \pm 0.7}$ & $51.38_{\, \pm 1.8}$ & $41.50_{\, \pm 1.0}$ & $45.09_{\, \pm 0.4}$ & $42.64_{\, \pm 2.6}$ \\
%         \midrule
%         Self-Certainty & \cellcolor{lightpurple5}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple3}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple7}{$75.0_{\, \pm 1.9}$} & \cellcolor{lightpurple2}{$88.93_{\, \pm 0.9}$} & \cellcolor{lightpurple5}{$44.58_{\, \pm 5.5}$} & \cellcolor{lightblue4}{$11.87_{\, \pm 0.7}$} & \cellcolor{lightblue5}{$53.87_{\, \pm 1.8}$} & \cellcolor{lightblue1}{$39.66_{\, \pm 1.0}$} & \cellcolor{lightblue5}{$43.89_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$41.98_{\, \pm 2.6}$} \\
%         Entropy & \cellcolor{lightpurple7}{$16.67_{\, \pm 6.9}$} & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple3}{$73.4_{\, \pm 2.0}$} & \cellcolor{lightpurple1}{$85.52_{\, \pm 1.0}$} & \cellcolor{lightpurple3}{$39.76_{\, \pm 5.4}$} & \cellcolor{lightblue6}{$15.68_{\, \pm 0.8}$} & \cellcolor{lightblue2}{$51.50_{\, \pm 1.8}$} & \cellcolor{lightblue2}{$40.25_{\, \pm 1.0}$} & \cellcolor{lightblue2}{$42.61_{\, \pm 0.4}$} & \cellcolor{tealgreen3}{$41.71_{\, \pm 2.8}$} \\
%         Majority-Voting & \cellcolor{lightpurple2}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple1}{$71.4_{\, \pm 2.0}$} & \cellcolor{lightpurple5}{$90.22_{\, \pm 0.8}$} & \cellcolor{lightpurple1}{$38.55_{\, \pm 5.3}$} & \cellcolor{lightblue7}{$18.37_{\, \pm 0.9}$} & \cellcolor{lightblue3}{$52.38_{\, \pm 1.8}$} & \cellcolor{lightblue4}{$42.72_{\, \pm 1.0}$} & \cellcolor{lightblue4}{$43.83_{\, \pm 0.4}$} & \cellcolor{tealgreen2}{$41.20_{\, \pm 2.4}$} \\
%         CoReward & \cellcolor{lightpurple2}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple5}{$74.0_{\, \pm 2.0}$} & \cellcolor{lightpurple6}{$90.52_{\, \pm 0.8}$} & \cellcolor{lightpurple1}{$38.55_{\, \pm 5.3}$} & \cellcolor{lightblue2}{$10.37_{\, \pm 0.6}$} & \cellcolor{lightblue7}{$57.25_{\, \pm 1.8}$} & \cellcolor{lightblue6}{$43.75_{\, \pm 1.0}$} & \cellcolor{lightblue1}{$42.08_{\, \pm 0.4}$} & \cellcolor{tealgreen1}{$41.09_{\, \pm 2.3}$} \\
%         LLM-KD & \cellcolor{lightpurple5}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$73.6_{\, \pm 2.0}$} & \cellcolor{lightpurple4}{$89.99_{\, \pm 0.8}$} & \cellcolor{lightpurple6}{$45.78_{\, \pm 5.5}$} & \cellcolor{lightblue1}{$8.09_{\, \pm 0.5}$} & \cellcolor{lightblue1}{$51.38_{\, \pm 1.8}$} & \cellcolor{lightblue5}{$43.09_{\, \pm 1.0}$} & \cellcolor{lightblue3}{$43.73_{\, \pm 0.4}$} & \cellcolor{tealgreen5}{$42.11_{\, \pm 2.7}$} \\
%         LLM-as-a-Judge  & \cellcolor{lightpurple2}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple3}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple2}{$72.2_{\, \pm 2.0}$} & \cellcolor{lightpurple3}{$89.61_{\, \pm 0.8}$} & \cellcolor{lightpurple4}{$42.17_{\, \pm 5.4}$} & \cellcolor{lightblue3}{$10.58_{\, \pm 0.6}$} & \cellcolor{lightblue4}{$53.00_{\, \pm 1.8}$} & \cellcolor{lightblue7}{$44.17_{\, \pm 1.0}$} & \cellcolor{lightblue6}{$48.67_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$41.90_{\, \pm 2.5}$} \\
%         \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple5}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple7}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple6}{$74.6_{\, \pm 1.9}$} & \cellcolor{lightpurple7}{$91.21_{\, \pm 0.8}$} & \cellcolor{lightpurple7}{$48.19_{\, \pm 5.5}$} & \cellcolor{lightblue5}{$14.69_{\, \pm 0.8}$} & \cellcolor{lightblue6}{$55.62_{\, \pm 1.8}$} & \cellcolor{lightblue3}{$41.51_{\, \pm 1.0}$} & \cellcolor{lightblue7}{$50.00_{\, \pm 0.4}$} & \cellcolor{tealgreen7}{$44.72_{\, \pm 2.8}$} \\

%         \bottomrule[1.6pt]
%     \end{tabular}}
% \end{table*}




\begin{table*}[!t]
    \centering
    \caption{RL performance (\%) on math reasoning benchmarks. Cell background colors indicate relative performance: darker colors denote better results within each model group.  
    }
    \renewcommand{\arraystretch}{1.05}
    \label{tab:main_math}
    % \vspace{1mm}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|rrcccrcccc}
    \toprule[1.6pt]
        \multirow{2}*{\textbf{Methods}} & \multicolumn{5}{c}{\textbf{Mathematics}} & \multicolumn{2}{c}{\textbf{Code}} & \textbf{Instruction} & \textbf{Multi-Task} & \multirow{2}*{\textbf{Average}} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10}

        ~ & \textbf{AIME24} & \textbf{AIME25} & \textbf{MATH500} & \textbf{GSM8K} & \textbf{AMC} & \textbf{LiveCode} & \textbf{CRUX} & \textbf{IFEval} & \textbf{MMLU-Pro} &  ~ \\
        \midrule
            \multicolumn{11}{c}{\textit{\textbf{Qwen3-1.7B-Base}}} \\ 
        \midrule

        Before RL & $6.67_{\, \pm 4.6}$ & $6.67_{\, \pm 4.6}$ & $45.8_{\, \pm 2.2}$ & $63.31_{\, \pm 1.3}$ & $26.51_{\, \pm 4.8}$ & $4.59_{\, \pm 0.4}$ & $7.12_{\, \pm 0.9}$ & $33.66_{\, \pm 1.0}$ & $33.60_{\, \pm 0.4}$ & $25.33_{\, \pm 2.3}$ \\
        GT-Reward & $10.00_{\, \pm 5.6}$ & $0.00_{\, \pm 0.0}$ & $68.2_{\, \pm 2.1}$ & $83.09_{\, \pm 1.0}$ & $34.94_{\, \pm 5.2}$ & $14.84_{\, \pm 0.9}$ & $33.75_{\, \pm 1.7}$ & $38.70_{\, \pm 1.0}$ & $39.43_{\, \pm 0.4}$ & $35.88_{\, \pm 2.0}$ \\
        \midrule
        Self-Certainty & \cellcolor{lightpurple3}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple1}{$57.2_{\, \pm 2.2}$} & \cellcolor{lightpurple1}{$74.68_{\, \pm 1.2}$} & \cellcolor{lightpurple1}{$26.51_{\, \pm 4.8}$} & \cellcolor{lightblue1}{$10.37_{\, \pm 0.7}$} & \cellcolor{lightblue1}{$19.00_{\, \pm 1.4}$} & \cellcolor{lightblue7}{$38.58_{\, \pm 1.0}$} & \cellcolor{lightblue2}{$35.28_{\, \pm 0.4}$} & \cellcolor{tealgreen1}{$30.18_{\, \pm 2.2}$} \\
        Entropy & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple4}{$65.2_{\, \pm 2.1}$} & \cellcolor{lightpurple2}{$79.98_{\, \pm 1.1}$} & \cellcolor{lightpurple3}{$32.53_{\, \pm 5.1}$} & \cellcolor{lightblue2}{$12.64_{\, \pm 0.8}$} & \cellcolor{lightblue2}{$31.00_{\, \pm 1.6}$} & \cellcolor{lightblue2}{$35.00_{\, \pm 1.0}$} & \cellcolor{lightblue4}{$37.01_{\, \pm 0.4}$} & \cellcolor{tealgreen3}{$34.08_{\, \pm 2.4}$} \\
        Majority-Voting & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple1}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple2}{$59.8_{\, \pm 2.2}$} & \cellcolor{lightpurple4}{$81.88_{\, \pm 1.1}$} & \cellcolor{lightpurple4}{$33.73_{\, \pm 5.2}$} & \cellcolor{lightblue5}{$14.29_{\, \pm 0.9}$} & \cellcolor{lightblue4}{$32.75_{\, \pm 1.7}$} & \cellcolor{lightblue5}{$37.16_{\, \pm 1.0}$} & \cellcolor{lightblue3}{$35.68_{\, \pm 0.4}$} & \cellcolor{tealgreen2}{$33.18_{\, \pm 1.8}$} \\
        CoReward & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple5}{$66.0_{\, \pm 2.1}$} & \cellcolor{lightpurple5}{$82.03_{\, \pm 1.1}$} & \cellcolor{lightpurple4}{$33.73_{\, \pm 5.2}$} & \cellcolor{lightblue4}{$14.27_{\, \pm 0.9}$} & \cellcolor{lightblue3}{$32.12_{\, \pm 1.6}$} & \cellcolor{lightblue6}{$37.28_{\, \pm 1.0}$} & \cellcolor{lightblue5}{$37.39_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$35.13_{\, \pm 2.4}$} \\
        LLM-KD & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple7}{$68.4_{\, \pm 2.1}$} & \cellcolor{lightpurple6}{$82.41_{\, \pm 1.1}$} & \cellcolor{lightpurple7}{$44.58_{\, \pm 5.5}$} & \cellcolor{lightblue3}{$14.05_{\, \pm 0.9}$} & \cellcolor{lightblue5}{$34.62_{\, \pm 1.7}$} & \cellcolor{lightblue1}{$34.65_{\, \pm 1.0}$} & \cellcolor{lightblue6}{$37.97_{\, \pm 0.4}$} & \cellcolor{tealgreen6}{$35.93_{\, \pm 2.1}$} \\
        LLM-as-a-Judge  & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple3}{$62.8_{\, \pm 2.2}$} & \cellcolor{lightpurple3}{$80.52_{\, \pm 1.1}$} & \cellcolor{lightpurple2}{$31.33_{\, \pm 5.1}$} & \cellcolor{lightblue6}{$14.33_{\, \pm 0.9}$} & \cellcolor{lightblue7}{$36.12_{\, \pm 1.7}$} & \cellcolor{lightblue3}{$36.28_{\, \pm 1.0}$} & \cellcolor{lightblue1}{$33.83_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$34.28_{\, \pm 2.4}$} \\
        \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple7}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple7}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple7}{$68.4_{\, \pm 2.1}$} & \cellcolor{lightpurple7}{$83.32_{\, \pm 1.0}$} & \cellcolor{lightpurple6}{$36.14_{\, \pm 5.3}$} & \cellcolor{lightblue7}{$14.54_{\, \pm 0.9}$} & \cellcolor{lightblue6}{$35.00_{\, \pm 1.7}$} & \cellcolor{lightblue4}{$36.55_{\, \pm 1.0}$} & \cellcolor{lightblue7}{$38.11_{\, \pm 0.4}$} & \cellcolor{tealgreen7}{$36.90_{\, \pm 2.6}$} \\
        \specialrule{1pt}{0.4ex}{0.4ex}
            \multicolumn{11}{c}{\textit{\textbf{Llama-3.2-3B-Instruct}}} \\ 
        \midrule

        Before RL & $3.33_{\, \pm 3.3}$ & $0.00_{\, \pm 0.0}$ & $42.8_{\, \pm 2.2}$ & $69.75_{\, \pm 1.3}$ & $13.25_{\, \pm 3.7}$ & $3.00_{\, \pm 0.4}$ & $25.50_{\, \pm 1.5}$ & $54.41_{\, \pm 1.1}$ & $32.01_{\, \pm 0.4}$ & $27.12_{\, \pm 1.6}$ \\
        GT-Reward & $13.33_{\, \pm 6.3}$ & $0.00_{\, \pm 0.0}$ & $48.0_{\, \pm 2.2}$ & $76.72_{\, \pm 1.2}$ & $22.89_{\, \pm 4.6}$ & $7.05_{\, \pm 0.6}$ & $32.62_{\, \pm 1.7}$ & $50.16_{\, \pm 1.1}$ & $34.26_{\, \pm 0.4}$ & $31.67_{\, \pm 2.0}$ \\
        \midrule
        Entropy & \cellcolor{lightpurple2}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple2}{$40.4_{\, \pm 2.2}$} & \cellcolor{lightpurple1}{$68.99_{\, \pm 1.3}$} & \cellcolor{lightpurple1}{$13.25_{\, \pm 3.7}$} & \cellcolor{lightblue2}{$5.38_{\, \pm 0.5}$} & \cellcolor{lightblue2}{$26.62_{\, \pm 1.6}$} & \cellcolor{lightblue7}{$54.24_{\, \pm 1.1}$} & \cellcolor{lightblue2}{$33.54_{\, \pm 0.4}$} & \cellcolor{tealgreen1}{$27.68_{\, \pm 1.7}$} \\
        Self-Certainty & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple1}{$40.2_{\, \pm 2.2}$} & \cellcolor{lightpurple2}{$74.07_{\, \pm 1.2}$} & \cellcolor{lightpurple2}{$16.87_{\, \pm 4.1}$} & \cellcolor{lightblue3}{$5.57_{\, \pm 0.6}$} & \cellcolor{lightblue1}{$22.75_{\, \pm 1.5}$} & \cellcolor{lightblue6}{$54.11_{\, \pm 1.1}$} & \cellcolor{lightblue6}{$34.42_{\, \pm 0.4}$} & \cellcolor{tealgreen2}{$27.92_{\, \pm 1.6}$} \\
        Majority-Voting & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple3}{$47.0_{\, \pm 2.2}$} & \cellcolor{lightpurple5}{$79.08_{\, \pm 1.1}$} & \cellcolor{lightpurple3}{$19.28_{\, \pm 4.3}$} & \cellcolor{lightblue7}{$8.11_{\, \pm 0.7}$} & \cellcolor{lightblue4}{$31.87_{\, \pm 1.6}$} & \cellcolor{lightblue1}{$48.36_{\, \pm 1.1}$} & \cellcolor{lightblue3}{$33.94_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$30.85_{\, \pm 1.9}$} \\
        CoReward & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple6}{$49.2_{\, \pm 2.2}$} & \cellcolor{lightpurple6}{$79.76_{\, \pm 1.1}$} & \cellcolor{lightpurple4}{$20.48_{\, \pm 4.4}$} & \cellcolor{lightblue3}{$5.57_{\, \pm 0.5}$} & \cellcolor{lightblue3}{$30.38_{\, \pm 1.6}$} & \cellcolor{lightblue4}{$50.46_{\, \pm 1.1}$} & \cellcolor{lightblue1}{$32.95_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$30.98_{\, \pm 1.9}$} \\
        LLM-KD & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple7}{$49.4_{\, \pm 2.2}$} & \cellcolor{lightpurple4}{$78.47_{\, \pm 1.1}$} & \cellcolor{lightpurple4}{$20.48_{\, \pm 4.4}$} & \cellcolor{lightblue6}{$7.55_{\, \pm 0.6}$} & \cellcolor{lightblue5}{$32.38_{\, \pm 1.6}$} & \cellcolor{lightblue2}{$49.06_{\, \pm 1.1}$} & \cellcolor{lightblue4}{$34.04_{\, \pm 0.4}$} & \cellcolor{tealgreen5}{$31.26_{\, \pm 1.9}$} \\
        LLM-as-a-Judge  & \cellcolor{lightpurple2}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple4}{$47.8_{\, \pm 2.2}$} & \cellcolor{lightpurple3}{$77.10_{\, \pm 1.2}$} & \cellcolor{lightpurple6}{$21.69_{\, \pm 4.5}$} & \cellcolor{lightblue1}{$3.96_{\, \pm 0.4}$} & \cellcolor{lightblue7}{$33.88_{\, \pm 1.7}$} & \cellcolor{lightblue5}{$51.46_{\, \pm 1.1}$} & \cellcolor{lightblue5}{$34.22_{\, \pm 0.4}$} & \cellcolor{tealgreen3}{$30.75_{\, \pm 1.8}$} \\
        \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple7}{$16.67_{\, \pm 6.9}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple5}{$49.0_{\, \pm 2.2}$} & \cellcolor{lightpurple7}{$80.74_{\, \pm 1.1}$} & \cellcolor{lightpurple7}{$24.10_{\, \pm 4.7}$} & \cellcolor{lightblue5}{$6.16_{\, \pm 0.6}$} & \cellcolor{lightblue6}{$32.62_{\, \pm 1.7}$} & \cellcolor{lightblue3}{$50.09_{\, \pm 1.1}$} & \cellcolor{lightblue7}{$34.54_{\, \pm 0.4}$} & \cellcolor{tealgreen7}{$32.66_{\, \pm 2.1}$} \\
        \specialrule{1pt}{0.4ex}{0.4ex}
            \multicolumn{11}{c}{\textit{\textbf{Qwen2.5-7B}}} \\ 
        \midrule

        Before RL & $3.33_{\, \pm 3.3}$ & $3.33_{\, \pm 3.3}$ & $49.2_{\, \pm 2.2}$ & $71.65_{\, \pm 1.2}$ & $20.48_{\, \pm 4.4}$ & $4.57_{\, \pm 0.4}$ & $28.00_{\, \pm 1.6}$ & $40.61_{\, \pm 1.0}$ & $44.03_{\, \pm 0.4}$ & $29.47_{\, \pm 2.0}$ \\
        GT-Reward & $13.33_{\, \pm 6.3}$ & $6.67_{\, \pm 4.6}$ & $76.4_{\, \pm 1.9}$ & $89.61_{\, \pm 0.8}$ & $46.99_{\, \pm 5.5}$ & $12.78_{\, \pm 0.7}$ & $51.38_{\, \pm 1.8}$ & $41.50_{\, \pm 1.0}$ & $45.09_{\, \pm 0.4}$ & $42.64_{\, \pm 2.6}$ \\
        \midrule
        Self-Certainty & \cellcolor{lightpurple5}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple3}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple7}{$75.0_{\, \pm 1.9}$} & \cellcolor{lightpurple2}{$88.93_{\, \pm 0.9}$} & \cellcolor{lightpurple5}{$44.58_{\, \pm 5.5}$} & \cellcolor{lightblue4}{$11.87_{\, \pm 0.7}$} & \cellcolor{lightblue5}{$53.87_{\, \pm 1.8}$} & \cellcolor{lightblue1}{$39.66_{\, \pm 1.0}$} & \cellcolor{lightblue5}{$43.89_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$41.98_{\, \pm 2.6}$} \\
        Entropy & \cellcolor{lightpurple7}{$16.67_{\, \pm 6.9}$} & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple3}{$73.4_{\, \pm 2.0}$} & \cellcolor{lightpurple1}{$85.52_{\, \pm 1.0}$} & \cellcolor{lightpurple3}{$39.76_{\, \pm 5.4}$} & \cellcolor{lightblue6}{$15.68_{\, \pm 0.8}$} & \cellcolor{lightblue2}{$51.50_{\, \pm 1.8}$} & \cellcolor{lightblue2}{$40.25_{\, \pm 1.0}$} & \cellcolor{lightblue2}{$42.61_{\, \pm 0.4}$} & \cellcolor{tealgreen3}{$41.71_{\, \pm 2.8}$} \\
        Majority-Voting & \cellcolor{lightpurple2}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple1}{$71.4_{\, \pm 2.0}$} & \cellcolor{lightpurple5}{$90.22_{\, \pm 0.8}$} & \cellcolor{lightpurple1}{$38.55_{\, \pm 5.3}$} & \cellcolor{lightblue7}{$18.37_{\, \pm 0.9}$} & \cellcolor{lightblue3}{$52.38_{\, \pm 1.8}$} & \cellcolor{lightblue4}{$42.72_{\, \pm 1.0}$} & \cellcolor{lightblue4}{$43.83_{\, \pm 0.4}$} & \cellcolor{tealgreen2}{$41.20_{\, \pm 2.4}$} \\
        CoReward & \cellcolor{lightpurple2}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple1}{$3.33_{\, \pm 3.3}$} & \cellcolor{lightpurple5}{$74.0_{\, \pm 2.0}$} & \cellcolor{lightpurple6}{$90.52_{\, \pm 0.8}$} & \cellcolor{lightpurple1}{$38.55_{\, \pm 5.3}$} & \cellcolor{lightblue2}{$10.37_{\, \pm 0.6}$} & \cellcolor{lightblue7}{$57.25_{\, \pm 1.8}$} & \cellcolor{lightblue6}{$43.75_{\, \pm 1.0}$} & \cellcolor{lightblue1}{$42.08_{\, \pm 0.4}$} & \cellcolor{tealgreen1}{$41.09_{\, \pm 2.3}$} \\
        LLM-KD & \cellcolor{lightpurple5}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple5}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple4}{$73.6_{\, \pm 2.0}$} & \cellcolor{lightpurple4}{$89.99_{\, \pm 0.8}$} & \cellcolor{lightpurple6}{$45.78_{\, \pm 5.5}$} & \cellcolor{lightblue1}{$8.09_{\, \pm 0.5}$} & \cellcolor{lightblue1}{$51.38_{\, \pm 1.8}$} & \cellcolor{lightblue5}{$43.09_{\, \pm 1.0}$} & \cellcolor{lightblue3}{$43.73_{\, \pm 0.4}$} & \cellcolor{tealgreen5}{$42.11_{\, \pm 2.7}$} \\
        LLM-as-a-Judge  & \cellcolor{lightpurple2}{$10.00_{\, \pm 5.6}$} & \cellcolor{lightpurple3}{$6.67_{\, \pm 4.6}$} & \cellcolor{lightpurple2}{$72.2_{\, \pm 2.0}$} & \cellcolor{lightpurple3}{$89.61_{\, \pm 0.8}$} & \cellcolor{lightpurple4}{$42.17_{\, \pm 5.4}$} & \cellcolor{lightblue3}{$10.58_{\, \pm 0.6}$} & \cellcolor{lightblue4}{$53.00_{\, \pm 1.8}$} & \cellcolor{lightblue7}{$44.17_{\, \pm 1.0}$} & \cellcolor{lightblue6}{$48.67_{\, \pm 0.4}$} & \cellcolor{tealgreen4}{$41.90_{\, \pm 2.5}$} \\
        \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple5}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple7}{$13.33_{\, \pm 6.3}$} & \cellcolor{lightpurple6}{$74.6_{\, \pm 1.9}$} & \cellcolor{lightpurple7}{$91.21_{\, \pm 0.8}$} & \cellcolor{lightpurple7}{$48.19_{\, \pm 5.5}$} & \cellcolor{lightblue5}{$14.69_{\, \pm 0.8}$} & \cellcolor{lightblue6}{$55.62_{\, \pm 1.8}$} & \cellcolor{lightblue3}{$41.51_{\, \pm 1.0}$} & \cellcolor{lightblue7}{$50.00_{\, \pm 0.4}$} & \cellcolor{tealgreen7}{$44.72_{\, \pm 2.8}$} \\

        \bottomrule[1.6pt]
    \end{tabular}}
\end{table*}


% 

% \begin{table*}[!t]
%     \centering
%     \caption{Main Results (\%) of \textit{RL performance} comparison on math reasoning benchmarks. Cell background colors indicate relative performance: darker colors denote better results within each model group.  
%     }
%     \renewcommand{\arraystretch}{1.05}
%     \label{tab:main_math}
%     % \vspace{2mm}
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{l|rrcccrcccc}
%     \toprule[1.6pt]
%         \multirow{2}*{\textbf{Methods}} & \multicolumn{5}{c}{\textbf{Mathematics}} & \multicolumn{2}{c}{\textbf{Code}} & \textbf{Instruction} & \textbf{Multi-Task} & \multirow{2}*{\textbf{Average}} \\ \cmidrule(lr){2-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9} \cmidrule(lr){10-10}

%         ~ & \textbf{AIME24} & \textbf{AIME25} & \textbf{MATH-500} & \textbf{GSM8K} & \textbf{AMC} & \textbf{LiveCode} & \textbf{CRUX} & \textbf{IFEval} & \textbf{MMLU-Pro} &  ~ \\
%         \midrule
%             \multicolumn{11}{c}{\textit{\textbf{Qwen3-1.7B-Base}}} \\ 
%         \midrule

%         Before RL & $6.67_{\, \pm 9.1}$ & $6.67_{\, \pm 9.1}$ & $45.8_{\, \pm 4.4}$ & $63.31_{\, \pm 2.6}$ & $26.51_{\, \pm 9.5}$ & $4.59_{\, \pm 0.8}$ & $7.12_{\, \pm 1.8}$ & $33.66_{\, \pm 1.9}$ & $33.60_{\, \pm 0.8}$ & $25.33_{\, \pm 4.4}$ \\
%         GT-Reward & $10.00_{\, \pm 10.9}$ & $0.00_{\, \pm 0.0}$ & $68.2_{\, \pm 4.1}$ & $83.09_{\, \pm 2.0}$ & $34.94_{\, \pm 10.3}$ & $14.84_{\, \pm 1.8}$ & $33.75_{\, \pm 3.3}$ & $38.70_{\, \pm 2.0}$ & $39.43_{\, \pm 0.8}$ & $35.88_{\, \pm 3.9}$ \\
%         \midrule
%         Self-Certainty & \cellcolor{lightpurple3}{$6.67_{\, \pm 9.1}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple1}{$57.2_{\, \pm 4.3}$} & \cellcolor{lightpurple1}{$74.68_{\, \pm 2.4}$} & \cellcolor{lightpurple1}{$26.51_{\, \pm 9.5}$} & \cellcolor{lightblue1}{$10.37_{\, \pm 1.4}$} & \cellcolor{lightblue1}{$19.00_{\, \pm 2.7}$} & \cellcolor{lightblue7}{$38.58_{\, \pm 2.0}$} & \cellcolor{lightblue2}{$35.28_{\, \pm 0.8}$} & \cellcolor{tealgreen1}{$30.18_{\, \pm 4.3}$} \\
%         Entropy & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple4}{$65.2_{\, \pm 4.2}$} & \cellcolor{lightpurple2}{$79.98_{\, \pm 2.2}$} & \cellcolor{lightpurple3}{$32.53_{\, \pm 10.1}$} & \cellcolor{lightblue2}{$12.64_{\, \pm 1.7}$} & \cellcolor{lightblue2}{$31.00_{\, \pm 3.2}$} & \cellcolor{lightblue2}{$35.00_{\, \pm 1.9}$} & \cellcolor{lightblue4}{$37.01_{\, \pm 0.8}$} & \cellcolor{tealgreen3}{$34.08_{\, \pm 4.6}$} \\
%         Majority-Voting & \cellcolor{lightpurple1}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple1}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple2}{$59.8_{\, \pm 4.3}$} & \cellcolor{lightpurple4}{$81.88_{\, \pm 2.1}$} & \cellcolor{lightpurple4}{$33.73_{\, \pm 10.2}$} & \cellcolor{lightblue5}{$14.29_{\, \pm 1.8}$} & \cellcolor{lightblue4}{$32.75_{\, \pm 3.3}$} & \cellcolor{lightblue5}{$37.16_{\, \pm 1.9}$} & \cellcolor{lightblue3}{$35.68_{\, \pm 0.8}$} & \cellcolor{tealgreen2}{$33.18_{\, \pm 3.4}$} \\
%         CoReward & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple5}{$66.0_{\, \pm 4.2}$} & \cellcolor{lightpurple5}{$82.03_{\, \pm 2.1}$} & \cellcolor{lightpurple4}{$33.73_{\, \pm 10.2}$} & \cellcolor{lightblue4}{$14.27_{\, \pm 1.8}$} & \cellcolor{lightblue3}{$32.12_{\, \pm 3.2}$} & \cellcolor{lightblue6}{$37.28_{\, \pm 2.0}$} & \cellcolor{lightblue5}{$37.39_{\, \pm 0.8}$} & \cellcolor{tealgreen4}{$35.13_{\, \pm 4.6}$} \\
%         LLM-KD & \cellcolor{lightpurple1}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple7}{$68.4_{\, \pm 4.1}$} & \cellcolor{lightpurple6}{$82.41_{\, \pm 2.1}$} & \cellcolor{lightpurple7}{$44.58_{\, \pm 10.7}$} & \cellcolor{lightblue3}{$14.05_{\, \pm 1.8}$} & \cellcolor{lightblue5}{$34.62_{\, \pm 3.3}$} & \cellcolor{lightblue1}{$34.65_{\, \pm 1.9}$} & \cellcolor{lightblue6}{$37.97_{\, \pm 0.8}$} & \cellcolor{tealgreen6}{$35.93_{\, \pm 4.2}$} \\
%         LLM-as-a-Judge  & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple4}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple3}{$62.8_{\, \pm 4.2}$} & \cellcolor{lightpurple3}{$80.52_{\, \pm 2.1}$} & \cellcolor{lightpurple2}{$31.33_{\, \pm 10.0}$} & \cellcolor{lightblue6}{$14.33_{\, \pm 1.8}$} & \cellcolor{lightblue7}{$36.12_{\, \pm 3.3}$} & \cellcolor{lightblue3}{$36.28_{\, \pm 1.9}$} & \cellcolor{lightblue1}{$33.83_{\, \pm 0.8}$} & \cellcolor{tealgreen4}{$34.28_{\, \pm 4.6}$} \\
%         \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple7}{$13.33_{\, \pm 12.4}$} & \cellcolor{lightpurple7}{$6.67_{\, \pm 9.1}$} & \cellcolor{lightpurple7}{$68.4_{\, \pm 4.1}$} & \cellcolor{lightpurple7}{$83.32_{\, \pm 2.0}$} & \cellcolor{lightpurple6}{$36.14_{\, \pm 10.3}$} & \cellcolor{lightblue7}{$14.54_{\, \pm 1.8}$} & \cellcolor{lightblue6}{$35.00_{\, \pm 3.3}$} & \cellcolor{lightblue4}{$36.55_{\, \pm 1.9}$} & \cellcolor{lightblue7}{$38.11_{\, \pm 0.8}$} & \cellcolor{tealgreen7}{$36.90_{\, \pm 5.1}$} \\
%         \specialrule{1pt}{0.4ex}{0.4ex}
%             \multicolumn{11}{c}{\textit{\textbf{Llama-3.2-3B-Instruct}}} \\ 
%         \midrule

%         Before RL & $3.33_{\, \pm 6.5}$ & $0.00_{\, \pm 0.0}$ & $42.8_{\, \pm 4.3}$ & $69.75_{\, \pm 2.5}$ & $13.25_{\, \pm 7.3}$ & $3.00_{\, \pm 0.8}$ & $25.50_{\, \pm 3.0}$ & $54.41_{\, \pm 2.1}$ & $32.01_{\, \pm 0.8}$ & $27.12_{\, \pm 3.0}$ \\
%         GT-Reward & $13.33_{\, \pm 12.4}$ & $0.00_{\, \pm 0.0}$ & $48.0_{\, \pm 4.4}$ & $76.72_{\, \pm 2.3}$ & $22.89_{\, \pm 9.0}$ & $7.05_{\, \pm 1.1}$ & $32.62_{\, \pm 3.3}$ & $50.16_{\, \pm 2.1}$ & $34.26_{\, \pm 0.8}$ & $31.67_{\, \pm 3.9}$ \\
%         \midrule
%         Entropy & \cellcolor{lightpurple2}{$6.67_{\, \pm 9.1}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple2}{$40.4_{\, \pm 4.3}$} & \cellcolor{lightpurple1}{$68.99_{\, \pm 2.5}$} & \cellcolor{lightpurple1}{$13.25_{\, \pm 7.3}$} & \cellcolor{lightblue2}{$5.38_{\, \pm 1.1}$} & \cellcolor{lightblue2}{$26.62_{\, \pm 3.1}$} & \cellcolor{lightblue7}{$54.24_{\, \pm 2.1}$} & \cellcolor{lightblue2}{$33.54_{\, \pm 0.8}$} & \cellcolor{tealgreen1}{$27.68_{\, \pm 3.4}$} \\
%         Self-Certainty & \cellcolor{lightpurple1}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple1}{$40.2_{\, \pm 4.3}$} & \cellcolor{lightpurple2}{$74.07_{\, \pm 2.4}$} & \cellcolor{lightpurple2}{$16.87_{\, \pm 8.1}$} & \cellcolor{lightblue3}{$5.57_{\, \pm 1.1}$} & \cellcolor{lightblue1}{$22.75_{\, \pm 2.9}$} & \cellcolor{lightblue6}{$54.11_{\, \pm 2.1}$} & \cellcolor{lightblue6}{$34.42_{\, \pm 0.8}$} & \cellcolor{tealgreen2}{$27.92_{\, \pm 3.1}$} \\
%         Majority-Voting & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple3}{$47.0_{\, \pm 4.4}$} & \cellcolor{lightpurple5}{$79.08_{\, \pm 2.2}$} & \cellcolor{lightpurple3}{$19.28_{\, \pm 8.5}$} & \cellcolor{lightblue7}{$8.11_{\, \pm 1.3}$} & \cellcolor{lightblue4}{$31.87_{\, \pm 3.2}$} & \cellcolor{lightblue1}{$48.36_{\, \pm 2.1}$} & \cellcolor{lightblue3}{$33.94_{\, \pm 0.8}$} & \cellcolor{tealgreen4}{$30.85_{\, \pm 3.7}$} \\
%         CoReward & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple6}{$49.2_{\, \pm 4.4}$} & \cellcolor{lightpurple6}{$79.76_{\, \pm 2.2}$} & \cellcolor{lightpurple4}{$20.48_{\, \pm 8.7}$} & \cellcolor{lightblue3}{$5.57_{\, \pm 1.0}$} & \cellcolor{lightblue3}{$30.38_{\, \pm 3.2}$} & \cellcolor{lightblue4}{$50.46_{\, \pm 2.1}$} & \cellcolor{lightblue1}{$32.95_{\, \pm 0.8}$} & \cellcolor{tealgreen4}{$30.98_{\, \pm 3.7}$} \\
%         LLM-KD & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple7}{$49.4_{\, \pm 4.4}$} & \cellcolor{lightpurple4}{$78.47_{\, \pm 2.2}$} & \cellcolor{lightpurple4}{$20.48_{\, \pm 8.7}$} & \cellcolor{lightblue6}{$7.55_{\, \pm 1.2}$} & \cellcolor{lightblue5}{$32.38_{\, \pm 3.2}$} & \cellcolor{lightblue2}{$49.06_{\, \pm 2.1}$} & \cellcolor{lightblue4}{$34.04_{\, \pm 0.8}$} & \cellcolor{tealgreen5}{$31.26_{\, \pm 3.7}$} \\
%         LLM-as-a-Judge  & \cellcolor{lightpurple2}{$6.67_{\, \pm 9.1}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple4}{$47.8_{\, \pm 4.4}$} & \cellcolor{lightpurple3}{$77.10_{\, \pm 2.3}$} & \cellcolor{lightpurple6}{$21.69_{\, \pm 8.9}$} & \cellcolor{lightblue1}{$3.96_{\, \pm 0.8}$} & \cellcolor{lightblue7}{$33.88_{\, \pm 3.3}$} & \cellcolor{lightblue5}{$51.46_{\, \pm 2.1}$} & \cellcolor{lightblue5}{$34.22_{\, \pm 0.8}$} & \cellcolor{tealgreen3}{$30.75_{\, \pm 3.5}$} \\
%         \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple7}{$16.67_{\, \pm 13.6}$} & \cellcolor{lightpurple2}{$0.00_{\, \pm 0.0}$} & \cellcolor{lightpurple5}{$49.0_{\, \pm 4.4}$} & \cellcolor{lightpurple7}{$80.74_{\, \pm 2.1}$} & \cellcolor{lightpurple7}{$24.10_{\, \pm 9.2}$} & \cellcolor{lightblue5}{$6.16_{\, \pm 1.1}$} & \cellcolor{lightblue6}{$32.62_{\, \pm 3.3}$} & \cellcolor{lightblue3}{$50.09_{\, \pm 2.1}$} & \cellcolor{lightblue7}{$34.54_{\, \pm 0.8}$} & \cellcolor{tealgreen7}{$32.66_{\, \pm 4.1}$} \\
%         \specialrule{1pt}{0.4ex}{0.4ex}
%             \multicolumn{11}{c}{\textit{\textbf{Qwen2.5-7B}}} \\ 
%         \midrule

%         Before RL & $3.33_{\, \pm 6.5}$ & $3.33_{\, \pm 6.5}$ & $49.2_{\, \pm 4.4}$ & $71.65_{\, \pm 2.4}$ & $20.48_{\, \pm 8.7}$ & $4.57_{\, \pm 0.7}$ & $28.00_{\, \pm 3.1}$ & $40.61_{\, \pm 2.0}$ & $44.03_{\, \pm 0.9}$ & $29.47_{\, \pm 3.9}$ \\
%         GT-Reward & $13.33_{\, \pm 12.4}$ & $6.67_{\, \pm 9.1}$ & $76.4_{\, \pm 3.7}$ & $89.61_{\, \pm 1.6}$ & $46.99_{\, \pm 10.7}$ & $12.78_{\, \pm 1.4}$ & $51.38_{\, \pm 3.5}$ & $41.50_{\, \pm 2.0}$ & $45.09_{\, \pm 0.9}$ & $42.64_{\, \pm 5.0}$ \\
%         \midrule
%         Self-Certainty & \cellcolor{lightpurple5}{$13.33_{\, \pm 12.4}$} & \cellcolor{lightpurple3}{$6.67_{\, \pm 9.1}$} & \cellcolor{lightpurple7}{$75.0_{\, \pm 3.8}$} & \cellcolor{lightpurple2}{$88.93_{\, \pm 1.7}$} & \cellcolor{lightpurple5}{$44.58_{\, \pm 10.7}$} & \cellcolor{lightblue4}{$11.87_{\, \pm 1.4}$} & \cellcolor{lightblue5}{$53.87_{\, \pm 3.4}$} & \cellcolor{lightblue1}{$39.66_{\, \pm 2.0}$} & \cellcolor{lightblue5}{$43.89_{\, \pm 0.9}$} & \cellcolor{tealgreen4}{$41.98_{\, \pm 5.0}$} \\
%         Entropy & \cellcolor{lightpurple7}{$16.67_{\, \pm 13.6}$} & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple3}{$73.4_{\, \pm 3.9}$} & \cellcolor{lightpurple1}{$85.52_{\, \pm 1.9}$} & \cellcolor{lightpurple3}{$39.76_{\, \pm 10.5}$} & \cellcolor{lightblue6}{$15.68_{\, \pm 1.6}$} & \cellcolor{lightblue2}{$51.50_{\, \pm 3.5}$} & \cellcolor{lightblue2}{$40.25_{\, \pm 2.0}$} & \cellcolor{lightblue2}{$42.61_{\, \pm 0.9}$} & \cellcolor{tealgreen3}{$41.71_{\, \pm 5.4}$} \\
%         Majority-Voting & \cellcolor{lightpurple2}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple1}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple1}{$71.4_{\, \pm 4.0}$} & \cellcolor{lightpurple5}{$90.22_{\, \pm 1.6}$} & \cellcolor{lightpurple1}{$38.55_{\, \pm 10.5}$} & \cellcolor{lightblue7}{$18.37_{\, \pm 1.8}$} & \cellcolor{lightblue3}{$52.38_{\, \pm 3.5}$} & \cellcolor{lightblue4}{$42.72_{\, \pm 2.0}$} & \cellcolor{lightblue4}{$43.83_{\, \pm 0.9}$} & \cellcolor{tealgreen2}{$41.20_{\, \pm 4.6}$} \\
%         CoReward & \cellcolor{lightpurple2}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple1}{$3.33_{\, \pm 6.5}$} & \cellcolor{lightpurple5}{$74.0_{\, \pm 3.8}$} & \cellcolor{lightpurple6}{$90.52_{\, \pm 1.6}$} & \cellcolor{lightpurple1}{$38.55_{\, \pm 10.5}$} & \cellcolor{lightblue2}{$10.37_{\, \pm 1.3}$} & \cellcolor{lightblue7}{$57.25_{\, \pm 3.4}$} & \cellcolor{lightblue6}{$43.75_{\, \pm 2.0}$} & \cellcolor{lightblue1}{$42.08_{\, \pm 0.9}$} & \cellcolor{tealgreen1}{$41.09_{\, \pm 4.5}$} \\
%         LLM-KD & \cellcolor{lightpurple5}{$13.33_{\, \pm 12.4}$} & \cellcolor{lightpurple5}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple4}{$73.6_{\, \pm 3.9}$} & \cellcolor{lightpurple4}{$89.99_{\, \pm 1.6}$} & \cellcolor{lightpurple6}{$45.78_{\, \pm 10.7}$} & \cellcolor{lightblue1}{$8.09_{\, \pm 1.0}$} & \cellcolor{lightblue1}{$51.38_{\, \pm 3.5}$} & \cellcolor{lightblue5}{$43.09_{\, \pm 2.0}$} & \cellcolor{lightblue3}{$43.73_{\, \pm 0.9}$} & \cellcolor{tealgreen5}{$42.11_{\, \pm 5.2}$} \\
%         LLM-as-a-Judge  & \cellcolor{lightpurple2}{$10.00_{\, \pm 10.9}$} & \cellcolor{lightpurple3}{$6.67_{\, \pm 9.1}$} & \cellcolor{lightpurple2}{$72.2_{\, \pm 3.9}$} & \cellcolor{lightpurple3}{$89.61_{\, \pm 1.6}$} & \cellcolor{lightpurple4}{$42.17_{\, \pm 10.6}$} & \cellcolor{lightblue3}{$10.58_{\, \pm 1.2}$} & \cellcolor{lightblue4}{$53.00_{\, \pm 3.4}$} & \cellcolor{lightblue7}{$44.17_{\, \pm 2.0}$} & \cellcolor{lightblue6}{$48.67_{\, \pm 0.9}$} & \cellcolor{tealgreen4}{$41.90_{\, \pm 4.9}$} \\
%         \textbf{JURY-RL (Ours)} & \cellcolor{lightpurple5}{$13.33_{\, \pm 12.4}$} & \cellcolor{lightpurple7}{$13.33_{\, \pm 12.4}$} & \cellcolor{lightpurple6}{$74.6_{\, \pm 3.8}$} & \cellcolor{lightpurple7}{$91.21_{\, \pm 1.5}$} & \cellcolor{lightpurple7}{$48.19_{\, \pm 10.7}$} & \cellcolor{lightblue5}{$14.69_{\, \pm 1.5}$} & \cellcolor{lightblue6}{$55.62_{\, \pm 3.4}$} & \cellcolor{lightblue3}{$41.51_{\, \pm 2.0}$} & \cellcolor{lightblue7}{$50.00_{\, \pm 0.9}$} & \cellcolor{tealgreen7}{$44.72_{\, \pm 5.4}$} \\

%         \bottomrule[1.6pt]
%     \end{tabular}}
% \end{table*}

